EICopilot: Search and Explore Enterprise Information over Large-scale Knowledge Graphs with LLM-driven Agents

The paper introduces EICopilot, an novel agent-based solution enhancing search and exploration of enterprise registration data within extensive online knowledge graphs like those detailing legal entities, registered capital, and major shareholders. Traditional methods necessitate text-based queries and manual subgraph explorations, often resulting in time-consuming processes. EICopilot, deployed as a chatbot via Baidu Enterprise Search, improves this landscape by utilizing Large Language Models (LLMs) to interpret natural language queries. This solution automatically generates and executes Gremlin scripts, providing efficient summaries of complex enterprise relationships. Distinct feature a data pre-processing pipeline that compiles and annotates representative queries into a vector database of examples for In-context learning (ICL), a comprehensive reasoning pipeline combining Chain-of-Thought with ICL to enhance Gremlin script generation for knowledge graph search and exploration, and a novel query masking strategy that improves intent recognition for heightened script accuracy. Empirical evaluations demonstrate the superior performance of EICopilot, including speed and accuracy, over baseline methods, with the \emph{Full Mask} variant achieving a syntax error rate reduction to as low as 10.00% and an execution correctness of up to 82.14%. These components collectively contribute to superior querying capabilities and summarization of intricate datasets, positioning EICopilot as a groundbreaking tool in the exploration and exploitation of large-scale knowledge graphs for enterprise information search.

==> relatedworks.tex <==
\section{Related Work}
In this section, we review the key areas relevant to our approach, focusing on Text2sql, Retrieval-Augmented Generation (RAG) \cite{gao2023retrieval}, and Information Retrieval \cite{zhu2023large}. These areas form the foundation of our methodology, leveraging advanced techniques to improve the querying and summarization of enterprise information from complex graph databases.


\subsection{Information Retrieval with LLMs}
Information retrieval aims at enabling efficient retrieval of information for user queries from large repositories. In general, users interact with the system by submitting queries in text form \cite{zhu2023large}. However, traditional approaches to information retrieval have several limitations. For instance, they often rely heavily on keyword matching, which can lead to issues with synonymy and polysemy, resulting in either too few or too many irrelevant results. Moreover, these systems typically do not incorporate contextual understanding, leading to suboptimal performance in complex query scenarios. The use of semantics for comprehensive enterprise data queries is one of the most promising areas for future innovation \cite{cagle2018ontology}. Due to the complex structure of enterprise information databases, simple keyword information retrieval cannot meet the increasingly complex query requirements. Its generalization is not enough, and manual intervention is often required in the data query stage. IR systems have long been divided into five main components: user modeling, indexing, matching/ranking, evaluation, and user interaction. By pre-training on large corpora and fine-tuning to human instructions, LLM has demonstrated remarkable abilities in language understanding, generation, interaction, and intellectual reasoning \cite{bubeck2023sparks}. Therefore, it is reasonable to expect that LLM will improve the effectiveness of the main components of the IR system in all aspects \cite{ai2023information}. Knowledge graphs (KGs) built on graph data structures are an effective way to solve this problem.


\subsection{ICL and RAG Techniques}
ICL refers to a model's ability to adapt its behavior based on inputs provided during inference, without undergoing weight updates, thereby enabling it to tackle tasks it wasn't explicitly trained on \cite{brown2020language}. This phenomenon was first observed in neural network architectures specifically designed for few-shot learning, where the model learns desired behaviors from just a few examples. In such scenarios, training involved shuffling the labels associated with input exemplars during each "episode" \cite{shin2022effect,lu2021fantastically}. Although ICL is effective, it often relies heavily on the quality of the presentation provided, which can result in suboptimal output. In addition, ICL may not have enough necessary information and prior knowledge to guide LLMs to generate the most accurate response. 

Recent studies have introduced retrieval-augmented generation (RAG) technology to improve the accuracy of traditional queries and address the hallucination problems of LLMs, where they generate fictitious information \cite{ding2024survey}. RAG enhances LLMs' performance by storing information in a database and retrieving relevant data as needed, mitigating the lack of answerable information \cite{borgeaud2022improving}. The RAG-LLMs framework includes retrieval, generation, and enhancement processes. Retrieval involves using a retriever to assess the relevance of documents to a query and improving retrieval quality via pre-retrieval and post-retrieval strategies \cite{lozano2023clinfo, wu2019scalable}. In the generation phase, a parameter-inaccessible generator produces responses using enhanced inputs without altering the model's internal structure \cite{achiam2023gpt, chen2021evaluating, ramos2003using}. Enhancement considers input, output, and intermediate layers of the generator, integrating retrieved documentation with original inputs (e.g., In-Context RALM, Atlas, and REPLUG) and incorporating retrieval results within the generative model \cite{poesia2022synchromesh, hofstatter2023fid, schick2024toolformer, borgeaud2022improving}. RAG is also employed in business information querying due to its ability to supplement information and boost generation performance.  



\subsection{Text2SQL Techniques}
The task of generating SQL from English queries, studied since the 1970s \cite{androutsopoulos1995natural}, has seen advancements focused on integrating table content. Notable works include NL2SQL-RULE \cite{guo2019content}, RATSQL \cite{wang2019rat}, and Photon \cite{zeng2020photon}. NL2SQL-RULE enhances BERT with mark vectors for question-token and table-header matching. Photon limits integration to exact matches in certain fields, whereas ColloQL embeds table content in BERT for enriched representations \cite{zeng2020photon}. TaBERT pre-trains text and table data jointly, outperforming standard models in tasks \cite{yin2020tabert}. The BIRD benchmark \cite{li2024can} emphasizes handling large databases and noisy data, offering a comprehensive test suite. Rebei's fine-tuning improves accuracy in retail-specific SQL dialects \cite{rebei2023finetuninglanguagemodelscontextspecific}. RAT-SQL uses a self-attention mechanism for schema encoding, excelling on the Spider dataset. SageCopilot \cite{liao2024towards} integrates LLMs for automating data science tasks and refining scripts, validated with real-world data. Deng et al. review the progress in Text-to-SQL and suggest future directions \cite{deng2022recent}.
Despite substantial progress in Text2SQL systems, current approaches continue to face significant challenges. These include difficulties in generalizing across diverse schema structures, inefficiencies in scaling to large and complex datasets, and limitations in handling noisy or incomplete data. Additionally, many models remain overly sensitive to slight variations in query phrasing, leading to inconsistent performance. Addressing these limitations is crucial for advancing the capabilities and robustness of Text-to-SQL systems.

\subsection{Discussions}
Our work advances beyond current approaches by addressing the traditional IR limitations of keyword dependence and contextual deficiency \cite{zhu2023large}. Unlike typical IR systems, \ours{} utilizes advanced LLMs pre-trained on large datasets and fine-tuned for human instructions \cite{bubeck2023sparks}, effectively enhancing semantic comprehension for complex enterprise queries and reducing manual intervention \cite{cagle2018ontology}. It builds on concepts like ICL and RAG, which respectively allow adaptation without weight updates \cite{brown2020language} and mitigate LLM hallucinations through retrieval \cite{ding2024survey}, by implementing dynamic integration for query pair generation \cite{gao2023retrieval}. The novel masking strategy further boosts example matching, improving accuracy in intent recognition—a key for complex query handling. Additionally, \ours{} tackles challenges in Text2SQL by generating Gremlin scripts and employing ICL to resolve schema discrepancies, promoting accurate SQL generation in large database contexts \cite{androutsopoulos1995natural}\cite{deng2022recent}. This positions \ours{} as a state-of-the-art solution in enterprise information retrieval and summarization.  

